Cooperative Relaying at Finite SNR -- Role of Quantize-Map-and-Forward

Quantize-Map-and-Forward (QMF) relaying has been shown to achieve the optimal diversity-multiplexing trade-off (DMT) for arbitrary slow fading full-duplex networks as well as for the single-relay half-duplex network. A key reason for this is that quantizing at the noise level suffices to achieve the cut-set bound approximately to within an additive gap, without any requirement of instantaneous channel state information (CSI). However, DMT only captures the high SNR performance and potentially, limited CSI at the relay can improve performance at moderate SNRs. In this work we propose an optimization framework for QMF relaying over slow fading channels. Focusing on vector Gaussian quantizers, we optimize the outage probability for the full-duplex and half-duplex single relay by finding the best quantization level and relay schedule according to the available CSI at the relays. For the N-relay diamond network, we derive an universal quantizer that sharpens the additive approximation gap of QMF from the conventional \Theta(N) bits/s/Hz to \Theta(log(N)) bits/s/Hz using only network topology information. Analytical solutions to channel-aware optimal quantizers for two-relay and symmetric N-relay diamond networks are also derived. In addition, we prove that suitable hybridizations of our optimized QMF schemes with Decode-Forward (DF) or Dynamic DF protocols provide significant finite SNR gains over the individual schemes.

==> App_Static.tex <==
%\subsection{Quantizer Optimization for the Full-Duplex Relay}

When the relay has access to the instantaneous channel gain realizations $h, g_1$ and $g_2$, it will choose a quantizer distortion $\Delta^*$ that maximizes $R_{\mbox{QMF}}(\Delta)$. Hence, the optimization problem can be stated as a $\max\min$ problem as follows:
\begin{equation*}
R_{\text{QMF}}^*=\max_{\Delta > 0}\lbp \left\lceil \min \lbp I_1, I_2 \rbp \right\rceil^+ \rbp
\end{equation*} and the optimizing $\Delta$ is denoted by $\Delta^*$.

We note that $I_1$ is \emph{monotonically decreasing} in $\Delta$ and $I_2$ is \emph{monotonically increasing} in $\Delta$. Also, at the boundary points of the admissible range of $\Delta$, we have,
\begin{align*}
I_1(0) = \lim_{\Delta \rightarrow 0^+} I_1&=\log \lp 1 + h^2 + g_2^2 \rp &
I_1(\infty) = \lim_{\Delta \rightarrow \infty} I_1&=\log \lp 1 + g_2^2 \rp\\
I_2(0) = \lim_{\Delta \rightarrow 0^+} I_2&=-\infty &
I_2(\infty) = \lim_{\Delta \rightarrow \infty} I_2&=\log \lp 1 + g_1^2 + g_2^2 \rp
\end{align*}

The properties $I_1 > 0 \quad \forall \Delta>0$, $I_2(0) < I_1(0)$ and $I_2(\infty) > I_1(\infty)$, together with the above mentioned monotonicity properties ensure that the optimum quantizer distortion is given by
\begin{equation*}
\Delta^* = \arg_{\Delta}\lbp I_1 = I_2 \rbp = \frac{1 + h^2 + g_2^2}{g_1^2}
\end{equation*}

%\subsection{Schedule Optimization for the Half-Duplex Relay}
%
%When the relay has access to the instantaneous channel realizations $h, g_1$ and $g_2$, it will choose a schedule $f$ that maximizes $\ol{C}_{hd}(f)$. Hence, the optimization problem can be stated as a $\max\min$ problem as follows:
%\begin{equation*}
%\ol{C}_{hd}^*=\max_{f \in  \lp 0, 1 \rp}\lbp \min \lbp C_{hd,1}(f), C_{hd,2}(f) \rbp \rbp
%\end{equation*} and the optimizing $f$ is denoted by $f^*$.
%
%We note that $C_{hd,1}$ is \emph{monotonically increasing} in $f$ and $C_{hd,2}$ is \emph{monotonically decreasing} in $f$. Also, at the boundary points of the admissible range of $f$, we have,
%\begin{align*}
%C_{hd,1}(0) = \lim_{f \rightarrow 0^+} C_{hd,1}&=\log \lp 1 + g_2^2 \rp\\
%C_{hd,1}(1) = \lim_{f \rightarrow \infty} C_{hd,1}&=\log \lp 1 + h^2 + g_2^2 \rp
%\end{align*} and
%\begin{align*}
%C_{hd,2}(0) = \lim_{f \rightarrow 0^+} C_{hd,2}&=\log \lp 1 + \lp g_1 + g_2 \rp^2 \rp \\
%C_{hd,2}(1) = \lim_{f \rightarrow \infty} C_{hd,2}&=\log \lp 1 + g_2^2 \rp
%\end{align*}
%
%The properties $C_{hd,1}(0) < C_{hd,2}(0)$ and $C_{hd,1}(1) > C_{hd,2}(1)$ together with the above mentioned monotonicity of $C_{hd,1}$ and $C_{hd,2}$ ensure that the optimum schedule is given by
%\begin{align*}
%f^* &= \arg_{f}\lbp C_{hd,1} = C_{hd,2} \rbp = \frac{\log \lp \frac{1 + \lp g_1 + g_2 \rp^2}{1 + g_2^2} \rp}{\log \lp \frac{\lp 1 + h^2 + g_2^2 \rp \lp 1 + \lp g_1 + g_2 \rp^2 \rp}{\lp 1 + g_2^2 \rp^2} \rp}
%\end{align*}


==> app_Pf_lem2_NRelay.tex <==
For $i \in [0:N-1]$,
\begin{align*}
R_i(\Delta) - R_{i+1}(\Delta) = 
\lbp\begin{array}{l}
\log \lbp \lp1 + \frac{(N-i)h^2}{1+\Delta}\rp\lp1+ig^2\rp\lp\frac{\Delta}{1+\Delta}\rp^i \rbp\\ 
- \log \lbp \lp1 + \frac{(N-i-1)h^2}{1+\Delta}\rp\lp1+(i+1)g^2\rp\lp\frac{\Delta}{1+\Delta}\rp^{i+1} \rbp
\end{array}\rbp
\end{align*}
The above can be simplified as,
\begin{align*}
R_i(\Delta) - R_{i+1}(\Delta) = 
\lbp\begin{array}{l}
\log \lp \frac{1+\Delta}{\Delta}\rp + \log \lp \frac{1 + \Delta + (N-i)h^2}{1 + \Delta + (N-i-1)h^2} \rp + \log \lp \frac{1 + ig^2}{1 + (i+1)g^2} \rp
\end{array}\rbp
\end{align*}
From the above, we note that for finite $h$ and $g$, $\lim_{\Delta\rightarrow 0}\lbp R_i(\Delta) - R_{i+1}(\Delta) \rbp = +\infty$ due to the presence of the term $\log \lp \frac{1+\Delta}{\Delta}\rp$ in the expression for $R_i(\Delta) - R_{i+1}(\Delta)$, which proves the lemma.


==> app_Pf_lem3_NRelay.tex <==
We define the sequence of polynomials $f_m(\Delta) = \frac{(1 +\Delta)^{m+2}}{\Delta^m}\lp 2^{R_{m+1}(\Delta)} - 2^{R_m(\Delta)} \rp $. Further, let $\Delta^{*}_m$ denote the unique positive root of $f_m(\Delta)$ (which is also the unique positive solution of $R_m(\Delta) = R_{m+1}(\Delta)$). Then, $\Delta^{*}_m$ satisfies
\begin{align*}
&g^2{\Delta^*_m}^2
+ \lp g^2 \lp 1 + (N-m)h^2 \rp - 1 - h^2 - g^2h^2 + 2mg^2 \rp{\Delta^*_m} 
- \lp 1+mg^2 \rp \lp 1 + (N-m)h^2 \rp\\
&= 0.
\end{align*}

For the required condition to hold true, i.e, $\Delta^{*}_m \leq \Delta^{*}_{m+1}$, we must have $f_{m+1}(\Delta^{*}_m) < 0$, since $R_{m+1}(\Delta) > R_{m+2}(\Delta)$ for $\Delta \in (0,\Delta^{*}_{m+1})$ by the preceding lemma. For $f_{m+1}(\Delta^{*}_m) < 0$, we obtain
\begin{align*}
\Delta^{*}_m \geq \frac{h^2\lp1 + (m+1)g^2\rp - g^2\lp1 + (N-m)h^2\rp}{g^2(2 + h^2)} = \Delta_t. %\mbox{ say.}
\end{align*}
What now remains to be shown in order for the lemma to hold is that $f_m(\Delta_t)<0$ for all values of $h,g,N$ and all $m \in [0:N-1]$. Substituting the value of $\Delta_t$, we obtain,
\begin{align*}
%\begin{array}{l}
f_m(\Delta_t) &= -\frac{h^6}{(2+h^2)^2}\lb \underbrace{m^2g^2 + m\lp2+(3-2N)g^2\rp+g^2(N-1)^2-(N-2)+\frac{1}{g^2}}_{\Gamma}\rb\\
&\quad - \frac{h^4}{(2+h^2)^2}\lb N+2(m+1)+g^2(N^2+2m-1)+\frac{2}{g^2}\rb\\
&\quad -\frac{h^2}{(2+h^2)^2}\lb2N+3+4m+g^2\lp4m^2+4m+(2N-1)\rp+\frac{2}{g^2}\rb\\
&\quad -\frac{1}{(2+h^2)^2}\lb2+g^2\rb.
%\end{array}
\end{align*}

From the above expression for $f_m(\Delta_t)$, it is clear that $\Gamma>0$ is a sufficient condition for $f_m(\Delta_t)<0$. $\Gamma$ can be viewed as a quadratic in $m$ with a discriminant $D_{\Gamma} = (5-4N)g^4+4(1-N)g^2$. Since the coefficient of $m^2$ is positive, the necessary and sufficient condition for $\Gamma>0,\ \forall m,g,h,N$ is that $D_{\Gamma}<0$, which is satisfied for $N \geq 2$. This concludes the proof of the lemma.

